Class-imbalanced Domain Adaptation: An Empirical Odyssey

Unsupervised domain adaptation is a promising way to generalize deep models to novel domains. However, the current literature assumes that the label distribution is domain-invariant and only aligns the feature distributions or vice versa. In this work, we explore the more realistic task of Class-imbalanced Domain Adaptation: How to align feature distributions across domains while the label distributions of the two domains are also different? Taking a practical step towards this problem, we constructed the first benchmark with 22 cross-domain tasks from 6real-image datasets. We conducted comprehensive experiments on 10 recent domain adaptation methods and find most of them are very fragile in the face of coexisting feature and label distribution shift. Towards a better solution, we further proposed a feature and label distribution CO-ALignment (COAL) model with a novel combination of existing ideas. COAL is empirically shown to outperform the most recent domain adaptation methods on our benchmarks. We believe the provided benchmarks, empirical analysis results, and the COAL baseline could stimulate and facilitate future research towards this important problem.

==> 3.2_PseudoCode.tex <==
\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line
\newcommand{\nosemic}{\renewcommand{\@endalgocfline}{\relax}}% Drop semi-colon ;
\newcommand{\dosemic}{\renewcommand{\@endalgocfline}{\algocf@endline}}% Reinstate semi-colon ;
\newcommand{\pushline}{\Indp}% Indent
\newcommand{\popline}{\Indm\dosemic}% Undent

\begin{algorithm}[t]
  \KwIn{$F$, $C$, $\mathcal{D}_S$, $\mathcal{D}_T$, $N_{iter}$, $N_{epoch}$, $N_{b}$, $k=k_{0}$}
  \KwOut{{$\hat{F}$}, {$\hat{C}$}}
  train $F$ and $C$ with $\mathcal{D}_S$ using Equation \ref{loss:supervise}\;
  \For{$i = 0, ..., N_{epoch}$}{
    \textbf{Step A}:\;
    $\quad$ compute $\hat{\mathcal{D}}_T=\{(x^t_i, \hat{y}^t_i, m_i)_{i=1}^{N_t}\}$ with $k$ as in Section \ref{method_PL}\;
    \textbf{Step B}:\;
      \For{$j = 0, ..., N_{iter}$}{
        randomly sample mini-batch: \\
        $\{(x^s_i, y^s_i)_{i=1}^{N_{b}}\} \in \mathcal{D}_S$, $ \{(x^t_i, \hat{y^t}_i, m_i)_{i=1}^{N_{b}}\} \in \hat{\mathcal{D}_T}$\;
        update $F$ and $C$ with Equation \ref{loss:minmax} \;
      }
    $k = \min(k + k_{step}, k_{max})$
  }
  \caption{Feature and Label Distribution CO-ALignment}
  \label{alg:main}
  \vspace{-0.2in}
\end{algorithm}


==> 4.4_VisDAResult.tex <==
\begin{table}[htbp]
 \renewcommand\arraystretch{0.8}
  \scriptsize
  \centering
  \begin{tabular}{l*{13}{p{0.54cm}<{\centering}}} 
    % {p{1.40cm}<{\centering}*{}{p{0.4cm}<{\centering}
  \toprule[1.2pt]
    Methods & plane & bcycl & bus & car & horse & knife & mcycl & person & plant & sktbrd & train & truck & MEAN  \\
    \midrule
    SourceOnly & 58.41 & 20.41 & 50.65 & \textbf{71.14} & 60.46 & 1.23 & 77.95 & 46.00 & 65.61 & 19.10 & 82.61 & 5.50   & 46.59  \\
    \midrule
    DAN & 75.96 & 45.48 & 12.99 & 32.78 & 82.51 & 17.89 & 66.53 & 44.83 & 71.50 & 60.07 & \textbf{94.46} & 6.62 & 50.97 \\
    JAN & 87.02 & 66.76 & 58.35 & 21.24 & \textbf{89.54} & 24.80 & 56.99 & 72.12 & 85.75 & 35.42 & 86.46 & 20.89 & 58.78 \\
    DANN & \textbf{87.98} & \textbf{72.89} & 71.52 & 24.51 & 84.31 & 8.94 & 46.78 & 75.63 & 87.75 & 55.21 & 81.69 & 16.31 & 59.46 \\
    BSP & 77.89 & 55.10 & 65.19 & 17.61 & 82.75 & 14.63 & 39.01 & 66.67 & 74.68 & 50.00 & 74.00 & 12.58 & 52.51 \\
    FDANN & 54.81 & 17.78 & 12.21 & 42.16 & 53.97 & \textbf{65.85} & 75.55 & 30.60 & 41.58 & 17.36 & 58.31 & 1.42 & 39.30 \\
    MCD & 64.83 & 40.70 & 79.97 & 60.59 & 83.42 & 39.26 & 88.29 & \textbf{71.86} & 78.81 & 65.92 & 82.14 & 5.98 & 63.48 \\
    PADA & 82.93 & 14.58 & 46.15 & 32.98 & 41.11 & 2.44 & 41.39 & 8.97 & 58.19 & 32.29 & 87.85 & 11.96 & 38.40 \\
    BBSL & 70.91 & 21.28 & 60.52 & 65.83 & 64.06 & 1.22 & 78.26 & 33.53 & \textbf{89.64} & 30.56 & 82.31 & 5.27 & 50.28 \\
    \midrule
    M3 & 80.53 & 69.68 & \textbf{81.39} & 57.54 & 48.08 & 32.93 & \textbf{89.48} & 65.11 & 75.15 & \textbf{66.67} & 81.39 & \textbf{39.46} & \textbf{65.62} \\
    \bottomrule[1.2pt]
    \end{tabular}%
    \caption{Per-class accuracy on VisDA dataset with RS-UT label shifts}
  \label{tab:visda}%
\end{table}%

==> 6.1_DigitResult.tex <==
\begin{table}[htbp]
 \renewcommand\arraystretch{1.0}
  \small
  \centering 
  \begin{tabular}{l*{5}{p{1.1cm}<{\centering}}}
  \toprule[1.2pt]
    Methods  & USPS$\rightarrow$MNIST& MNIST$\rightarrow$USPS 
          & SVHN$\rightarrow$MNIST& SynD$\rightarrow$SVHN & AVG  \\
    \midrule
    Source Only & 71.49$\pm$0.08 & 84.73$\pm$1.34 & 56.95$\pm$1.52 & 86.33$\pm$0.56 & 76.00  \\
    \midrule
    FDANN (2019) & 72.13$\pm$1.88 & 87.30$\pm$0.99 & 34.16$\pm$1.64 & 80.77$\pm$1.45 & 67.41  \\
    BBSE (2018) & 79.42$\pm$3.04 & 74.07$\pm$3.56 & 53.73$\pm$3.19 & 87.14$\pm$0.88 & 71.65  \\
    PADA (2018) & 73.07$\pm$0.13 & 81.39$\pm$0.11 & 56.82$\pm$0.97 & 85.88$\pm$0.35 & 74.70  \\
    JAN (2017)& 87.69$\pm$0.51 & 93.93$\pm$0.34 & 56.00$\pm$4.30 & 82.65$\pm$3.02 & 77.53  \\
    DAN (2015)& 83.09$\pm$2.10 & 86.16$\pm$0.49 & 63.42$\pm$2.08 & 86.48$\pm$0.97 & 78.69  \\
    BSP (2019)& 83.33$\pm$1.77 & 89.21$\pm$1.44 & 63.31$\pm$2.43 & 93.24$\pm$0.53 & 81.92  \\
    DANN (2015)& 83.92$\pm$1.19 & 90.29$\pm$0.94 & 68.96$\pm$3.73 & 93.43$\pm$0.36 & 84.23  \\
    MCD & \textbf{97.53$\pm$0.04} & \textbf{96.86$\pm$0.60} & \textbf{88.47$\pm$1.96} & \textbf{96.82$\pm$0.32} & \textbf{94.92} \\
    \midrule
    COAL (Ours) & \underline{92.87$\pm$0.60} & \underline{95.40$\pm$0.59} & \underline{82.01$\pm$2.36} & \underline{96.39$\pm$0.26} & \underline{91.27}  \\
    
    \bottomrule[1.2pt]
    \end{tabular}%
    \caption{Class-balanced accuracy on Digit dataset with BS-BT label shifts}
    \label{tab:digit_BSBT}%
\end{table}%

==> 6.2_OfficeHomeResult.tex <==
\begin{table}[htbp]
 \renewcommand\arraystretch{1.0}
  \scriptsize
%   \small
  \centering
  \begin{tabular}{l*{7}{p{1.2cm}<{\centering}}} 
  \toprule[1.2pt]
    Methods  & Rw$\rightarrow$Pr & Rw$\rightarrow$Cl 
          & Pr$\rightarrow$Rw & Pr$\rightarrow$Cl & Cl$\rightarrow$Rw & Cl$\rightarrow$Pr &  AVG  \\                  
    \midrule
    Source Only & 72.91  & 39.21  & 69.84  & 38.16  & 56.06  & 54.08  & 55.04  \\
    \midrule
    PADA & 64.44  & 33.89  & 59.21  & 30.35  & 41.92  & 41.19  & 45.17  \\
    BBSE & 64.25  & 34.85  & 63.56  & 34.19  & 40.57  & 38.57  & 46.00  \\
    BSP & 72.85  & \textbf{50.29} & 69.35  & 25.20  & 34.31  & 31.92  & 47.32  \\
    MCD & 68.76  & 37.14  & 66.78  & 36.31  & 51.77  & 48.50  & 51.54  \\
    DAN & 71.67  & 38.35  & 67.42  & 36.07  & 55.48  & 53.25  & 53.71  \\
    FDANN & 71.20  & 39.11  & 67.30  & 33.86  & \underline{60.85}  & 53.64  & 54.33  \\
    JAN & 66.69  & 42.28  & 69.61  & 38.65  & 59.42  & \underline{57.19}  & 55.64  \\
    DANN & \underline{74.70}  & 47.10  & \underline{70.07}  & \underline{39.35}  & 60.56  & 54.88  & \underline{57.78}  \\
    \midrule
    COAL & \textbf{77.44} & \underline{47.42}  & \textbf{71.23} & \textbf{42.87} & \textbf{63.46} & \textbf{61.24} & \textbf{60.61} \\
    \bottomrule[1.2pt]
    \end{tabular}%
    \caption{Class-balanced accuracy on Office-Home dataset with BS-BT label shifts}
  \label{tab:OH_BSBT}%
\end{table}%

==> 6.3_VisDAResult.tex <==
\begin{table}[htbp]
 \renewcommand\arraystretch{0.8}
  \scriptsize
  \centering
  \begin{tabular}{l*{13}{p{0.54cm}<{\centering}}} 
    % {p{1.40cm}<{\centering}*{}{p{0.4cm}<{\centering}
  \toprule[1.2pt]
    Methods & plane & bcycl & bus & car & horse & knife & mcycl & person & plant & sktbrd & train & trunk & MEAN  \\
    \midrule
    \multicolumn{14}{c}{BS-BT} \\
    \midrule
    \midrule
    SourceOnly & 51.42  & 24.91  & 59.52  & 64.68  & 65.99  & 4.80  & 77.21  & 40.42  & 61.38  & 21.07  & 83.78  & 5.81  & 46.75  \\
    \midrule
    DAN & 69.77 & 37.24 & 70.29 & 51.09 & 78.27 & 40.07 & 73.52 & 59.37 & 75.63 & 38.00 & \textbf{86.46} & 14.20 & 57.83 \\
    JAN & 85.19 & 80.70 & 70.44 & 47.40 & \textbf{91.86} & 64.83 & 76.86 & 70.89 & 86.65 & 55.03 & 74.43 & 40.53 & 70.40 \\
    DANN & 88.67 & 80.34 & 68.67 & 55.89 & 88.73 & 41.18 & 82.47 & 74.08 & 84.98 & \textbf{68.37} & 72.71 & 34.72 & 70.07 \\
    BSP & \textbf{90.14} & \textbf{83.48} & 70.84 & 60.03 & 89.24 & 51.84 & 83.17 & \multicolumn{1}{r}{\textbf{75.29}} & 86.70 & 67.96 & 79.23 & \textbf{40.83} & \textbf{73.23} \\
    FDANN & 86.00 & 7.48 & \textbf{84.28} & 56.29 & 73.12 & \textbf{92.93} & 85.04 & 66.30 & 62.13 & 9.25 & 76.15 & 2.93 & 58.49 \\
    MCD & 88.74 & 66.06 & 83.35 & 67.72 & 88.36 & 9.78 & \textbf{86.86} & 66.52 & 73.44 & 85.36 & 77.46 & 13.08 & 67.23 \\
    PADA & 66.94 & 8.29 & 64.48 & 44.52 & 25.21 & 2.02 & 61.95 & 6.77 & 76.95 & 25.82 & 75.09 & 2.68 & 38.39 \\
    BBSE & 61.07 & 14.35 & 57.10 & \textbf{75.64} & 67.56 & 3.59 & 82.26 & 28.15 & 76.04 & 24.00 & 79.74 & 1.01 & 47.54 \\
    \midrule
    M3 & 83.77 & 59.68 & 79.94 & 69.83 & 84.89 & 34.26 & 86.56 & 72.51 & \textbf{86.91} & 61.55 & 78.07 & 40.07 & 69.84 \\
    \bottomrule[1.2pt]
    \end{tabular}%
    \caption{Per-class accuracy on VisDA dataset}
  \label{tab:visda}%
\end{table}%

==> tmp.tex <==
88.12 + 93.04 + 65.67 + 59.81 + 73.46 + 73.65 + 69.90 + 87.71 
